Learning Robust Real-World Dexterous Grasping Policies via Implicit Shape Augmentation

Dexterous robotic hands have the capability to interact with a wide variety of household objects to perform tasks like grasping. However, learning robust real world grasping policies for arbitrary objects has proven challenging due to the difficulty of generating high quality training data. In this work, we propose a learning system (ISAGrasp) for leveraging a small number of human demonstrations to bootstrap the generation of a much larger dataset containing successful grasps on a variety of novel objects. Our key insight is to use a correspondence-aware implicit generative model to deform object meshes and demonstrated human grasps in order to generate a diverse dataset of novel objects and successful grasps for supervised learning, while maintaining semantic realism. We use this dataset to train a robust grasping policy in simulation which can be deployed in the real world. We demonstrate grasping performance with a four-fingered Allegro hand in both simulation and the real world, and show this method can handle entirely new semantic classes and achieve a 79% success rate on grasping unseen objects in the real world.

==> texs/limitations.tex <==
\section{Limitations}
\label{sec:limitations}
% \begin{enumerate} moving to appendix
%     \item \textbf{Poor performance on challenging objects:} it’s more challenging for our policy to succeed when the object is large (e.g. cracker box lying on the table Appendix Figure 12a) or too flat (scissors in Appendix Figure 12b)).  Since our shape augmentation is built on dexYCB dataset, if the test object is too different from the training objects, or requires a more specific way of grasping (e.g. Eagle with two wings: Appendix Figure 12c). The shape augmentation also does not cover objects of widely varying scales. 
%     \item \textbf{Real world experiments:} The method assumes access to a fairly complete point cloud. It will not succeed in scenarios with heavy amounts of occlusion or noise in the point clouds. 
%     \item \textbf{Functional grasping:} Currently the method does not do dexterous and functional grasps, and is only designed to lift the object. The utility of a dexterous hand is perhaps best utilized with functional grasps, but the current system does not optimize for this directly. 
%     \item \textbf{Accounting for kinematics:} The current system does not account for the kinematics of potentially hitting the table when the hand is mounted on a full arm setup. This should be accounted for as we build on this work in the future. 
% \end{enumerate}
